Tailored Primitive Initialization is the Secret Key to Reinforcement Learning

Reinforcement learning (RL) has emerged as a powerful paradigm for enhancing the reasoning capabilities of large language models (LLMs). While RL has demonstrated substantial performance gains, it still faces key challenges, including low sampling efficiency and a strong dependence on model initialization: some models achieve rapid improvements with minimal RL steps, while others require significant training data to make progress. In this work, we investigate these challenges through the lens of reasoning token coverage and argue that initializing LLMs with diverse, high-quality reasoning primitives is essential for achieving stable and sample-efficient RL training. We propose Tailor, a finetuning pipeline that automatically discovers and curates novel reasoning primitives, thereby expanding the coverage of reasoning-state distributions before RL. Extensive experiments on mathematical and logical reasoning benchmarks demonstrate that Tailor generates more diverse and higher-quality warm-start data, resulting in higher downstream RL performance.

==> example_prompt/iGSM_prompt_example.tex <==
\begin{tcolorbox}[
colframe=darkgray, % Dark grey frame color
boxrule=0.2pt, % Frame thickness
colback=lightgray!20, %
arc=3pt, % Rounded corners
% fontupper=\small,
breakable,
halign=left
]
\textbf{iGSM Example prompt 1}: \\
Problem-Solving Instructions for Robust Reasoning\\
1. Define Variables and Equations:\\   
- List every entity and attribute mentioned in the query.\\   
- Assign a unique variable to each quantity.\\   
- Translate all given statements into equations using these variables.\\
2. Prioritize Independent Variables:\\   
- Solve variables with direct numerical assignments first (e.g., constants like `X = 5`).\\   
- Substitute these values into the dependent equations immediately.\\
3. \textcolor{red}{Build Dependency Graphs:}\\   
- For each unsolved variable, list all equations where it appears.\\   
- \textcolor{red}{Identify the simplest equation to resolve next (e.g., least dependencies).}\\
4. \textcolor{red}{Solve Step-by-Step:}\\   
- Proceed incrementally, substituting known values into dependent equations.\\   
5. \textcolor{red}{Validate Intermediate Results:}\\   
- \textcolor{red}{Recompute critical steps to verify consistency.}\\   
- Flag contradictions for re-evaluation.\\
6. \textcolor{red}{Target-Focused Resolution:}\\   
- \textcolor{red}{Clearly state the goal variable.}\\   
- Back-substitute from the goal to ensure all required variables are resolved.\\
7. Final Answer:\\   
- Conclude with a boxed numerical answer (`boxed\{N\}`) supported by the validated reasoning chain.\\
Note: All variables are solvable. 
\end{tcolorbox}

\begin{tcolorbox}[
colframe=darkgray, % Dark grey frame color
boxrule=0.2pt, % Frame thickness
colback=lightgray!20, %
arc=3pt, % Rounded corners
% fontupper=\small,
breakable,
halign=left
]
\textbf{iGSM Example prompt 2}: \\
Instructions for Solving the Problem:  \\
1. Define All Variables Explicitly:  \\   
- Assign variables to each entity and relationship mentioned, \textcolor{blue}{including composite terms (e.g., "Enclosure" = sum of sub-components).}  \\   
- Label all variables clearly (e.g., ( X\_{Store} ) for "X at Store").  \\
2. Translate Statements into Equations:  \\   
- Convert every given statement into a mathematical equation, \textcolor{blue}{even if it seems redundant.}  \\   
- Preserve all operations (sums, differences, multipliers) exactly as stated.  \\
3. Substitute Known Values Early:  \\   
- Substitute fixed values (e.g., "equals 9") immediately to simplify equations.  \\   
- Do not assume unconstrained variables are zero unless explicitly stated.  \\
4. Explore Indirect Relationships:  \\   
- Track how variables influence others indirectly (e.g., if ( A = B + C ) and ( B ) depends on ( D ), express ( A ) in terms of ( D )).  \\   
- {If a variable’s value is unresolved, check if it can be expressed in terms of other known variables.}  \\
5. Self-Correct for Consistency:  \\   
- If equations lead to contradictions (e.g., ( 0 = 1 )), revisit earlier steps to identify missed relationships or incorrect assumptions.  \\  
- \textcolor{blue}{Verify that all given statements are fully utilized in the solution.}  \\
6. Conclude Rigorously:  \\   
- Ensure every step logically follows from the previous ones.  \\   
- \textcolor{blue}{If ambiguity remains, exhaustively test plausible interpretations to understand the problem and conditions (e.g., "Enclosure" as a sum) to arrive at a valid answer.}
\end{tcolorbox}


